The Thermodynamic Costs of Simple Linear Regression

The construction of models from data is a significant contributor to the energetic costs of computation. Because of this, understanding how foundational thermodynamic bounds apply to modeling algorithms will be increasingly important. Here, we study the thermodynamic costs of a basic and fundamental modeling algorithm: simple linear regression. Following Landauer, we approximate the thermodynamic lower bound on irreversibly performing both exact linear regression and linear regression via stochastic gradient descent as implemented on floating-point numbers. From this, we derive energycost aware scaling laws for the optimal dataset size for training a linear regression model given a generalization error dependent demand for inference. Additionally, we discuss a method to lower bound the entropy production from the mismatch cost for algorithms with continuous input variables.

==> defs.tex <==
% organization
\newcommand{\bracket}[1]{\left[ #1 \right]}
\newcommand{\curly}[1]{\left\{ #1 \right\}}
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\abs}[1]{\left| #1 \right|}

% algebra
\newcommand{\R}[1]{\mathbb{R}^{#1}}
\newcommand{\N}[1]{\mathbb{N}^{#1}}
\newcommand{\Z}[1]{\mathbb{Z}^{#1}}
\newcommand{\C}[1]{\mathbb{C}^{#1}}
\newcommand{\K}[1]{\mathbb{K}^{#1}}
\newcommand{\Sym}[1]{\mathbb{S}^{#1}}
\newcommand{\norm}[2]{\left|\left| #1 \right|\right|_{#2}}
\newcommand{\innprod}[2]{\left\langle #1, #2 \right\rangle}

% probability
\newcommand{\Esub}[2]{\mathbb{E}_{#2}\left[ #1 \right]}
\newcommand{\E}[1]{\mathbb{E}\left[ #1 \right]}
\newcommand{\prob}[1]{\mathbb{P}\left( #1 \right)}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}} % independence symbol
\newcommand{\indic}[1]{\mathbbm{1}_{\left\{#1\right\}}} %indicator function
\newcommand{\iid}{\stackrel{iid}{\sim}} % iid


% pdfs and pmfs
\newcommand{\gauss}[2]{\mathcal{N}\paren{#1, #2}}
\newcommand{\bern}[1]{\mathrm{Ber}\paren{#1}}
\newcommand{\bin}[2]{\mathrm{Bin}\paren{#1, #2}}
\newcommand{\pois}[1]{\mathrm{Poisson}\paren{#1}}
\newcommand{\unif}[2]{\mathrm{Unif}\paren{#1, #2}}
\newcommand{\geo}[1]{\mathrm{Geometric}\paren{#1}}
\newcommand{\expon}[1]{\mathrm{Exp}\paren{#1}}
\newcommand{\hypgeo}[4]{\mathrm{HypGeo}\paren{#1, #2, #3, #4}}
% info theory
\newcommand{\alphx}{\mathcal{X}}
\newcommand{\alphy}{\mathcal{Y}}
\newcommand{\mutual}[2]{I\paren{#1;#2}}
\newcommand{\condmutual}[3]{I\paren{#1;#2|#3}}
\newcommand{\ent}[1]{H\paren{#1}}
\newcommand{\condent}[2]{H\paren{#1|#2}}
\newcommand{\jointent}[2]{H\paren{#1,#2}}
\newcommand{\relent}[2]{D\paren{#1||#2}}


%calculus
\newcommand{\del}[2]{\frac{\partial #1}{\partial #2}}


% % organization
% \newcommand{\bracket}[1]{\left[ #1 \right]}
% \newcommand{\paren}[1]{\left( #1 \right)}
% \newcommand{\abs}[1]{\left| #1 \right|}

% % algebra
% \newcommand{\R}[1]{\mathbb{R}^{#1}}
% \newcommand{\N}[1]{\mathbb{N}^{#1}}
% \newcommand{\Z}[1]{\mathbb{Z}^{#1}}
% \newcommand{\C}[1]{\mathbb{C}^{#1}}
% \newcommand{\K}[1]{\mathbb{K}^{#1}}
% \newcommand{\Sym}[1]{\mathbb{S}^{#1}}
% \newcommand{\norm}[2]{\left|\left| #1 \right|\right|_{#2}}
% \newcommand{\innprod}[2]{\left\langle #1, #2 \right\rangle}

% % probability
% \newcommand{\Esub}[2]{\mathbb{E}_{#2}\left[ #1 \right]}
% \newcommand{\E}[1]{\mathbb{E}\left[ #1 \right]}
% \newcommand{\prob}[1]{\mathbb{P}\left( #1 \right)}
% \newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
% \def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}} % independence symbol
% \newcommand{\indic}[1]{\mathbbm{1}_{\left\{#1\right\}}} %indicator function
% % pdfs and pmfs
% \newcommand{\gauss}[2]{\mathcal{N}\paren{#1, #2}}
% \newcommand{\bern}[1]{\mathrm{Ber}\paren{#1}}
% \newcommand{\bin}[2]{\mathrm{Bin}\paren{#1, #2}}
% \newcommand{\pois}[1]{\mathrm{Poisson}\paren{#1}}
% \newcommand{\unif}[2]{\mathrm{Unif}\paren{#1, #2}}
% \newcommand{\geo}[1]{\mathrm{Geometric}\paren{#1}}
% \newcommand{\expon}[1]{\mathrm{Exp}\paren{#1}}
% \newcommand{\hypgeo}[4]{\mathrm{HypGeo}\paren{#1, #2, #3, #4}}
% % info theory
% \newcommand{\alphx}{\mathcal{X}}
% \newcommand{\alphy}{\mathcal{Y}}
% \newcommand{\mutual}[2]{I\paren{#1;#2}}
% \newcommand{\condmutual}[3]{I\paren{#1;#2|#3}}
% \newcommand{\ent}[1]{H\paren{#1}}
% \newcommand{\condent}[2]{H\paren{#1|#2}}
% \newcommand{\jointent}[2]{H\paren{#1,#2}}
% \newcommand{\relent}[2]{D\paren{#1||#2}}


% %calculus
% \newcommand{\del}[2]{\frac{\partial #1}{\partial #2}}

